Lifetime-Limited Interrogation of Two Independent ${}^{27}\textrm{Al}^{+}$ Clocks Using Correlation Spectroscopy

Laser decoherence limits the stability of optical clocks by broadening the observable resonance linewidths and adding noise during the dead time between clock probes. Correlation spectroscopy avoids these limitations by measuring correlated atomic transitions between two ensembles, which provides a frequency difference measurement independent of laser noise. Here, we apply this technique to perform stability measurements between two independent clocks based on the $^1S_0\leftrightarrow{}^3P_0$ transition in $^{27}$Al$^+$. By stabilizing the dominant sources of differential phase noise between the two clocks, we observe coherence between them during synchronous Ramsey interrogations as long as 8 s at a frequency of $1.12\times10^{15}$ Hz. The observed contrast in the correlation spectroscopy signal is consistent with the 20.6 s $^3P_0$ state lifetime and supports a measurement instability of $(1.8\pm0.5)\times 10^{-16}/\sqrt{\tau/\textrm{s}}$ for averaging periods longer than the probe duration when deadtime is negligible.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
